Discussing the Spectrum of Physics-Enhanced Machine Learning; a Survey on Structural Mechanics Applications

The intersection of physics and machine learning has given rise to the physics-enhanced machine learning (PEML) paradigm, aiming to improve the capabilities and reduce the individual shortcomings of data- or physics-only methods. In this paper, the spectrum of physics-enhanced machine learning methods, expressed across the defining axes of physics and data, is discussed by engaging in a comprehensive exploration of its characteristics, usage, and motivations. In doing so, we present a survey of recent applications and developments of PEML techniques, revealing the potency of PEML in addressing complex challenges. We further demonstrate application of select such schemes on the simple working example of a single degree-of-freedom Duffing oscillator, which allows to highlight the individual characteristics and motivations of different `genres' of PEML approaches. To promote collaboration and transparency, and to provide practical examples for the reader, the code generating these working examples is provided alongside this paper. As a foundational contribution, this paper underscores the significance of PEML in pushing the boundaries of scientific and engineering research, underpinned by the synergy of physical insights and machine learning capabilities.

==> figures/arb_nn_topo.tex <==
\begin{tikzpicture}[x=2.2cm,y=1.4cm]
      \message{^^JNeural network, shifted}
      \readlist\Nnod{2,3,3,3,2} % array of number of nodes per layer
      \readlist\Nstr{n,m,m,m,k} % array of string number of nodes per layer
      \readlist\Cstr{\strut x,a^{(\prev)},a^{(\prev)},a^{(\prev)},y} % array of coefficient symbol per layer
      \def\yshift{0.5} % shift last node for dots
      
      \message{^^J  Layer}
      \foreachitem \N \in \Nnod{ % loop over layers
        \def\lay{\Ncnt} % alias of index of current layer
        \pgfmathsetmacro\prev{int(\Ncnt-1)} % number of previous layer
        \message{\lay,}
        \foreach \i [evaluate={\c=int(\i==\N); \y=\N/2-\i-\c*\yshift;
                     \index=(\i<\N?int(\i):"\Nstr[\lay]");
                     \x=\lay; \n=\nstyle;}] in {1,...,\N}{ % loop over nodes
          % NODES
          \node[node \n] (N\lay-\i) at (\x,\y) {$\Cstr[\lay]_{\index}$};
          
          % CONNECTIONS
          \ifnum\lay>1 % connect to previous layer
            \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
              \draw[connect] (N\prev-\j) -- (N\lay-\i);
            }
          \fi % else: nothing to connect first layer
          
        }
        \path (N\lay-\N) --++ (0,1+\yshift) node[midway,scale=1.5] {$\vdots$};
      }
      
      % LABELS
      \node[above=5,align=center,black!60!black] at (N1-1.90) {input\\[-0.2em]layer};
      \node[above=2,align=center,black!60!black] at (N3-1.90) {hidden layers};
      \node[above=10,align=center,black!60!black] at (N\Nnodlen-1.90) {output\\[-0.2em]layer};
      
\end{tikzpicture}

==> figures/paper_layout.tex <==
\begin{tikzpicture}[
    theme/.style={rectangle, draw, fill=black!10},
    spectrum/.style={rectangle, draw, left color=black!20, right color=white},
    method/.style={rectangle, draw, top color=white, bottom color=black!10, align=left},
    section/.style={rectangle, draw, fill=white, align=left},
    subsection/.style={grow=down, anchor=west, edge from parent path={(\tikzparentnode.south west) |- (\tikzchildnode.west)}},
    first/.style={level distance=6ex},
    second/.style={level distance=12ex},
    third/.style={level distance=18ex},
    level 1/.style={sibling distance=14em}]

    % Theme
    \coordinate
        child[grow=up] {node[theme,anchor=center]{Physics-Enhanced Machine Learning}}
        % child[grow=down, level distance=0ex] {node[spectrum, anchor=center] {}}
    [edge from parent fork down]
    % Sections and subsections
    child{node[section] {Forward Modelling/Simulation}
        child[subsection, first] {node[method, xshift=-13ex]{Reduction methods}}
        child[subsection, second] {node[method, xshift=-13ex]{Indirect fusion of physics}}
        child[subsection, third] {node[method, xshift=-13ex]{PINNs for FM}}}
    child{node[section] {Data-Driven Models}
        child[subsection, first] {node[method, xshift=-8ex]{Bayesian Logic}}
        child[subsection, second] {node[method, xshift=-8ex]{Equation Discovery}}}
    child{node[section] {Physics-Guided Learners}
        child[subsection, first] {node[method, xshift=-10ex]{Constrained GPs}}
        child[subsection, second] {node[method, xshift=-10ex]{PINNs}}};


\end{tikzpicture}
